Language-Image Models with 3D Understanding

Multi-modal large language models (MLLMs) have shown incredible capabilities in a variety of 2D vision and language tasks. We extend MLLMs' perceptual capabilities to ground and reason about images in 3-dimensional space. To that end, we first develop a large-scale pre-training dataset for 2D and 3D called LV3D by combining multiple existing 2D and 3D recognition datasets under a common task formulation: as multi-turn question-answering. Next, we introduce a new MLLM named Cube-LLM and pre-train it on LV3D. We show that pure data scaling makes a strong 3D perception capability without 3D specific architectural design or training objective. Cube-LLM exhibits intriguing properties similar to LLMs: (1) Cube-LLM can apply chain-of-thought prompting to improve 3D understanding from 2D context information. (2) Cube-LLM can follow complex and diverse instructions and adapt to versatile input and output formats. (3) Cube-LLM can be visually prompted such as 2D box or a set of candidate 3D boxes from specialists. Our experiments on outdoor benchmarks demonstrate that Cube-LLM significantly outperforms existing baselines by 21.3 points of AP-BEV on the Talk2Car dataset for 3D grounded reasoning and 17.7 points on the DriveLM dataset for complex reasoning about driving scenarios, respectively. Cube-LLM also shows competitive results in general MLLM benchmarks such as refCOCO for 2D grounding with (87.0) average score, as well as visual question answering benchmarks such as VQAv2, GQA, SQA, POPE, etc. for complex reasoning. Our project is available at https://janghyuncho.github.io/Cube-LLM.

==> sections/0_abstract.tex <==
\begin{abstract}
Multi-modal large language models (MLLMs) have shown incredible capabilities in a variety of 2D vision and language tasks.
We extend \mmfm{}s' perceptual capabilities to ground and reason about images in 3-dimensional space. 
To that end, we first develop a large-scale pretraining dataset for 2D and 3D called \dataset{} by combining multiple existing 2D and 3D recognition datasets under a common task formulation: as multi-turn question-answering.
Next, we introduce a new \mmfm{} named \ours and pre-train it on \dataset{}. 
We show that pure data scaling makes a strong 3D perception capability without 3D specific architectural design or training objective. 
\ours exhibits intriguing properties similar to LLMs: (1) \ours can apply chain-of-thought prompting to improve 3D understanding from 2D context information.
(2) \ours can follow complex and diverse instructions and adapt to versatile input and output formats. 
(3) \ours can be visually prompted such as 2D box or a set of candidate 3D boxes from specialists.
Our experiments demonstrate that \ours\footnote{Project repository:  \href{https://anonymous.4open.science/r/cubellm-E84E}{https://anonymous.4open.science/r/cubellm-E84E}.} significantly outperforms existing baselines by 14.8\% of AP$_{\text{BEV}}$ on the \ttc dataset for 3D grounded reasoning and 21.6\% of score on the \dLM dataset for complex reasoning, respectively. (\todo{add indoor and VLM benchmark results})

\keywords{Multi-modal Large Language Models \and 3D Scene Understanding \and Foundation Models \and Autonomous Driving}
\end{abstract}

==> sections/0_abstract_vicho.tex <==
\begin{abstract}
Multi-modal large language models (\mmfm{}s) have demonstrated incredible capabilities in a variety of language and 2D vision tasks through large-scale pre-training. 
However, their effectiveness diminishes when directly applied to 3D tasks, due to the limited coverage of internet-scale pre-training data for 3D reasoning.
% In this work, we argue that scaling up 3D data for pre-training is essential for adapting \mmfm{}s to 3D reasoning.
% and show significant performance improvement on the 3D grounding and 3D QA task.
To bridge this gap, in this work we develop a large-scale 3D vision-language QA dataset \dataset{} by amalgamating multiple 2D and 3D datasets and standardizing their sensor configurations.
% in order to pre-train \mmfm{}s to enhance its 3D reasoning capability. 
We additionally introduce a versatile framework \boris{for ...} named \ours and pre-train it on this dataset. Recognizing the complexity of direct 3D reasoning from 2D image data, \ours utilizes chain-of-thought (CoT) reasoning to facilitate 3D understanding from 2D context information. To further enhance its performance, \ours incorporates predictions from specialist models and employs an iterative approach to progressively increase input resolution during training, enabling more effective long-range reasoning.
% Additionally, we highlight the importance of resolution in long-range reasoning tasks and adopt an iterative approach to progressively increase input resolution during training, which significantly enhances model performance. 
% Our approach allows the injection of predictions from any specialist models to further improve performance. 
Our experiments on the \ttc and \dLM datasets demonstrate that \ours significantly outperforms existing baselines by 7 points of ?? and X points \yy{Vincent to fill them in} of ??, respectively. 
% This paper not only studies the significance of data scaling in 3D task performance but also offers a framework for enhancing 3D grounding and reasoning capabilities in autonomous driving and robotics.
  \keywords{Vision-Language Models \and 3D Scene Understanding \and Foundation Models \and Autonomous Driving}
\end{abstract}

==> sections/1_introduction_v2.tex <==
\section{Introduction}
\label{sec:intro}




Internet-scale visual data have brought forth the advent of multi-modal large language models (MLLMs). 
Rich and diverse visual supervision aligns pre-trained large language models with billions of parameters to visual modality. 
The best MLLMs can recognize, understand, and reason about images and videos far better than any of specially designed architectures and algorithms~\cite{gpt4_V,team2023gemini}. 
% \todo{What application? Why we need? Cite some papers that explains this.}
The decades worth of computer vision datasets  ---image classification, captioning, object detection, grounding, document parsing, optical character recognition (OCR)--- fuels the powerful MLLMs through jointly training as a {next token prediction} task. 
Introducing the ability to ``ground'' in 2-dimensional space (\emph{image coordinates}) bridges the low-level perception to high-level reasoning about visual input, much like human cognition. 
However, one critical difference is that we perceive the world in 3-dimensional space (\emph{view coordinates}). 
This 3-dimensional grounding allows us to perceive and reason about the visual input closer to the actual world, which the current state of MLLMs has not explored yet. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/teaser_v3.pdf}
    \caption{
    \ours and 3D-grounded reasoning. The task requires a model to understand the input text prompt (e.g., ``\textit{Turn left once that Audi passes.''}) and ground it in 3-dimensional space. \todo{indoor and outdoor visualization here instead?}
    }
    \label{fig:teaser-figure}
    % \vspace{-0.5cm}
\end{figure}

In this work, our goal is to develop a framework to train a MLLM capable of reasoning in both 2D and 3D spaces. 
We demonstrate that pure data scaling can achieve our goal without any 3D specific architectural design or training objective. 
We instead focus on careful data curation to address one question: \emph{what tasks will induce 2D to 3D generalization?} 
To this end, we introduce a large scale language-image pretraining dataset for 2D and 3D, called LV3D. 
We start with combining a diverse collection of 2D and 3D vision datasets for indoors and outdoors and standardize labels to follow the consistent format across datasets.
We blend in the vision datasets with instruction-following data of MLLM training as a series of question-answer pairs ($\S$~\ref{sec:data_scale}). 
Next, we augment our blended datasets by {decomposing} the vision labels into easier tasks (\emph{e.g., 3D box $\rightarrow$ 2D point, depth, size, orientation}).
This trains our model to adapt to versatile input and output format, and connect the underlying structure of 2D and 3D ($\S$~\ref{sec:task_scale}). 
% Furthermore, we directly induce 2D to 3D generalization by mixing in ``step-by-step'' question-answer pairs. 
% That is, we enquire easier question (\emph{e.g., 2D box}) and follow with harder ones (\emph{e.g., 3D box}) or prompt with a number of candidate answers (\emph{e.g., other bounding boxes}) to reduce the task difficulty ($\S$~\ref{sec:v_cot}). 
Most importantly, we mix in a series of QA pairs about an object for ``step-by-step'' reasoning, from easier (\emph{e.g., 2D box}) to harder (\emph{e.g., 3D box}) task.
This directly induces 2D to 3D generalization due to autoregressive nature of MLLMs ($\S$~\ref{sec:v_cot}).
Finally, we train a MLLM on LV3D as a single ``next token prediction'' task, called \ours ($\S$~\ref{sec:arch}). 

\ours exhibits a number of intriguing properties.
First, \ours can self-improve its 3D reasoning performance by prompting with its own 2D predictions.
This \emph{visual chain-of-thought reasoning} resembles the well-known behavior of LLMs~\cite{wei2022chain}. 
Second, \ours can adapt to versatile input and output formats and questions, which follows \emph{instruction following} ability of LLMs. 
Finally, \ours can be \emph{prompted} with any specialist models for any additional modalities (\emph{e.g., LiDAR}) by simply adding their predictions to the question. 
% \todo{talk about scaling}
\ours shows remarkable improvement with data-scaling in both 2D and 3D, for indoor and outdoor scenes grounding as well as complex reasoning tasks such as in driving scenarios. 

We evaluate our model's performance in both 3D grounding and 3D reasoning tasks on various driving datasets as well as a standard \mmfm{} benchmark, and show qualitative results in 3D grounding in non-driving scenes. 
For 3D grounding on the \ttc dataset~\cite{deruyttere2019talk2car}, \ours surpasses the baselines by 14.8\% in Bird's Eye View (BEV) AP (57.5 vs 50.1) and by 13.0\% in 3D AP (51.3 vs 45.4).
Additionally, our training framework improves the performance of \ours on the \dLM~\cite{sima2023drivelm} dataset, nearly doubling the performance in the BEV AP (66.0 vs 33.2) for 3D grounding and the overall score (39.4 vs 32.4) for complex reasoning, compared to directly \dLM baseline~\cite{sima2023drivelm}.
\todo{indoor and VLM results.}
% \todo{Qualitative experiments show that \ours outperforms alternative approaches in visual grounding beyond driving scenes.
% A joint 2D and 3D grounding model is generally better able to disambiguate spatial references.}


==> sections/1_introduction_vicho.tex <==
\section{Introduction}
\label{sec:intro}

Object recognition is almost perfectly divided into 2D recognition~\cite{} and 3D recognition~\cite{}.
Smaller, and often specialized datasets are required for accurate 3D recognition~\cite{}.
While large and diverse internet-scale recognition datasets provide the data, labels, and benchmarks for two dimensional recognition~\cite{}.
Internet-scale recognition datasets have brought forth the advent of multi-modal large language models (\mmfm{}s) with remarkable performance in 2D vision~\cite{}.
These models, often comprising billions of parameters, are pre-trained on massive datasets that encompass various modalities such as vision and language. 
By learning rich representations and cross-modal alignments from such heterogeneous data at internet scale, \mmfm{}s have demonstrated notable success in 2D image understanding tasks such as visual question answering, image captioning, and zero-shot transfer learning. 
Despite these successes, existing \mmfm{} works have predominantly focused on 2D vision and language tasks, and there has been limited exploration in 3D reasoning and scene understanding.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/teaser_v3.pdf}
    \caption{
    \ours and 3D-grounded reasoning. The task requires a model to understand the input text prompt (e.g., ``\textit{Turn left once that Audi passes.''}) and ground it in 3-dimensional space. 
    }
    \label{fig:teaser-figure}
    % \vspace{-0.5cm}
\end{figure}

To address the gap, we present \ours, a \mmfm{} that is capable of reasoning in both 2D and 3D spaces. 
We combine a diverse collection of 2D and 3D datasets for indoors and outdoors, which we call \dataset{}, and develop a framework to effectively scale up training for \mmfm{}. 
Our framework includes careful data curation and standardization to blend in with the existing instruction-following data for \mmfm{} training. 
We leverage existing labels in \dataset{} to train \ours for versatile input and output format, which improves understanding of the underlying structure of 2D and 3D reasoning. 
We show that \ours exhibits enhanced 3D reasoning performance when prompted with its own 2D predictions. We call this process \emph{visual chain-of-thought prompting} (VCoT), which is similar to chain-of-thought prompting in LLMs~\cite{wei2022chain} similar in spirit to~\cite{chen2023measuring} but in the context of 3D perception.
% \yue{have prior works done this before? If so, we might want to highlight the difference.}. 
Furthermore, we allow our model to incorporate the predictions of any specialist models as a system prompt. 
This alleviates the problem of 3D localization.
% \yue{what does this mean? maybe we can just say 3D localization?} and further improve the 3D localization. 
Our final model shows remarkable improvement in 3D reasoning. 

We evaluate our model's performance in both 3D grounding and 3D reasoning tasks on various driving datasets as well as a standard \mmfm{} benchmark, and show qualitative results in 3D grounding in non-driving scenes. 
For 3D grounding on the \ttc dataset~\cite{deruyttere2019talk2car}, \ours surpasses the baselines by 14.8\% in Bird's Eye View (BEV) AP (57.5 vs 50.1) and by 13.0\% in 3D AP (51.3 vs 45.4).
% Additionally, our training framework improves the performance of \ours for 3D grounding on \dLM, nearly doubling the performance in the BEV AP (66.0 vs 33.2), compared to directly finetuning LLaVA-1.5.  
% Finally, we demonstrate that \ours improves complex reasoning in \dLM QA benchmark, improving $7$  score from \dLM and 3.3 from LLaVA-1.5 (our base model).
Additionally, our training framework improves the performance of \ours on the \dLM~\cite{sima2023drivelm} dataset, nearly doubling the performance in the BEV AP (66.0 vs 33.2) for 3D grounding and the overall score (39.4 vs 32.4) for complex reasoning, compared to directly \dLM baseline~\cite{sima2023drivelm}.
\todo{Qualitative experiments show that \ours outperforms alternative approaches in visual grounding beyond driving scenes.
A joint 2D and 3D grounding model is generally better able to disambiguate spatial references.}

% In this paper, we expand \mmfm{}s' capabilities for 3D reasoning, specifically focusing on AV applications. 
% We construct a large-scale 3D visual-language pretraining dataset (\dataset{}) by standardizing numerous 2D and 3D datasets in indoors and outdoors, applying heuristics to generate diverse grounding tasks for \mmfm{} pretraining to improve 3D grounding and reasoning.
    % \item Visual Chain-of-Thought Prompting to connect 2D semantic reasoning with 3D scene geometry understanding for enhanced 3D grounding, employing high-resolution finetuning to boost overall performance significantly.
    % \item A model-agnostic method for injecting specialist models to utilize diverse input modalities effectively.
    % \item Evaluations on talk2car and Drive-LM for both 3D grounding and reasoning, achieving significant improvements over baselines by 7 and X points respectively.

% \boris{everything after here is quite detailed for an introduction and should be moved to method or even experimental sections.}

% An immediate and straightforward approach for adapting these models is to fine-tune them on tasks of 3D grounding or 3D question answering. 
% Instead, we argue there is a need for a methodological shift in adapting existing \mmfm{}s for 3D reasoning tasks.

% To validate our hypothesis, we first developed a large-scale 3D vision-language pre-training dataset that integrates object grounding tasks across both 2D and 3D domains. Specifically, our dataset is built on top of the Omni3D dataset~\cite{brazil2023omni3d}, which encompasses a diverse set of indoor and outdoor scenes, originally curated for 3D object detection tasks. \yy{We also includes 3D data from nuScenes, right?}
% To tailor the dataset for \mmfm{}s pre-training, we generate an extensive set of 3D question-answering pairs for object grounding by leveraging the human annotations from 3D detections \yy{correct it if this is wrong}, which significantly enhances the model's capabilities in aligning 3D information with natural language.
% , particularly in comprehending depth. 
% Additionally, we show our \mmfm{}s demonstrate favorable scaling laws with respect to the dataset size. 
% Our dataset is also augmented with a variety of large-scale 2D grounding datasets such as COCO~\cite{lin2014microsoft}, refCOCO~\cite{refcoco}, and Objects365~\cite{o365}, to improve the model's ability to generalize across various scenes and foster a more robust understanding of both 2D and 3D contexts. 

% While our dataset integrates both 2D and 3D grounding data, the predominance of 2D data means the model is naturally more adept at 2D grounding tasks. \yy{Correct this if it is wrong}
% To ease the difficulty of directly reasoning in 3D and fully leverage the model's well-trained 2D reasoning capability, we introduce a Visual Chain-of-Thought Prompting to improve 3D grounding result. 
% CoT first estimates the bounding box on 2D images based on the language question, then prompts the model with the predicted 2D bounding box to estimate the corresponding 3D bounding box. 
% By decomposing the complex 3D grounding task into more manageable sub-tasks of 2D semantic reasoning followed by 3D depth estimation, we facilitate a more effective use of the model's 2D proficiency to enhance its understanding of 3D spaces.
% Additionally, we underscore the significance of high image resolution in improving the accuracy of long-range depth estimation, which is crucial for precise 3D grounding.
% Our training approach involves an initial pre-training and fine-tuning phase using low-resolution images, followed by further fine-tuning on high-resolution images.
% These two techniques yield consistent performance improvement on both 3D grounding and QA tasks.

% To expand the input modalities, we propose a model-agnostic approach that utilizes predictions from specialized models utilizing different modality, \eg, LiDAR-based 3D object detection models.
% The predictions from specialized models serve as supplementary information to the original question for 3D grounding. 
% We train the model with the ground truth of the specialized task and incorporate specialized models' output during interference, ensuring it remains independent of any specific models.

% We evaluate our model's performance in both 3D grounding and 3D reasoning on various autonomous driving datasets as well as standard \mmfm{} benchmarks. 
% In the case of 3D grounding, our evaluation on the \ttc dataset~\cite{deruyttere2019talk2car} shows that our model surpasses the baseline models by 7 points in Bird's Eye View (BEV) accuracy and by 5 points in 3D\yc{It's hard to tell the improvement without knowing the baseline performance}. Additionally, we have adapted the \dLM model for 2D grounding to 3D and evaluated its performance, where it exceeds the LLaVA-1.5 fine-tuning baseline by X points. Regarding 3D reasoning, our analysis on \dLM demonstrates that our model achieves an improvement of X points over the baseline. \yc{I think evaluation-wise we might need to associate some takeaways to make this sound more exciting}


==> sections/1_intruction.tex <==
\section{Introduction}
\label{sec:intro}
% Autonomous driving and embodied AI have seen remarkable progress in recent years.  Despite this progress, maintaining safety remains a significant challenge, especially when handling rare situations, commonly known as corner cases. 
% These cases pose a serious risk to safety but are difficult to gather due to their rarity in the long tail distribution. However, humans possess an innate ability to recognize and navigate these rare scenarios using common sense. Integrating this human-like common sense into autonomous systems has the potential to markedly enhance their safety and reliability.


% \yy{I feel we need a more concrete example.}
% - Autonomous driving is advancing with remarkable progress, but we are still far from building driving system that can drive with versatile and generalizable 3D reasoning, that can really understand the nuance intents and interactions between human drivers and other traffic paticipants in the 3D scene.
% Autonomous driving has made remarkable progress in recent years, with advancements in perception, planning, and control enabling increasingly sophisticated self-driving capabilities. 
% However, despite these strides, we are still far from building driving systems that can operate with the versatile and generalizable reasoning capabilities in 3D that characterizes human driving, \eg, understand the nuanced intentions and interactions between human drivers and other traffic participants and plan the route neither too conservative nor too aggressive. 
% Such sophisticate 3D reasoning remains elusive for current autonomous driving systems.

% XW: merged two paragraph into one as the majority of the text was too verbose previously

\boris{A critical challenge preventing the widespread deployment of autonomous vehicles (AVs) is the scale to which they must generalize. In AV perception, for example, each region of the world may have unique road layouts, vehicle types, or weather patterns, among other factors, which complicate the generalization of learning-based 3D object detectors or trackers. Accordingly, developing versatile models for 3D perception and scene understanding is essential for AV generalization. However, naively scaling existing models by collecting labeled driving data from a wide variety of geographies is costly, necessitating more efficient solutions.}

Concurrently, the advent of multi-modal large language models (\mmfm{}s) \boris{good reference is \url{https://arxiv.org/abs/2401.13601}} has brought forth remarkable breakthroughs in 2D vision performance.
% Developing versatile models for 3D scene understanding is essential for intelligent systems such as autonomous vehicles, yet it still presents significant challenges. 
% Concurrently, in the realm of 2D vision domains, we are witnessing remarkable breakthroughs with the advent of multi-modal large language models (\mmfm{}s) 
These models, often comprising billions of parameters, are pre-trained on massive datasets that encompass various modalities such as vision and language. By learning rich representations and cross-modal alignments from such heterogeneous data at internet scale, \mmfm{}s have demonstrated notable success in 2D image understanding tasks such as visual question answering, image captioning, and zero-shot transfer learning. Despite these successes, existing \mmfm{} works have predominantly focused on 2D vision and language tasks, and there has been limited exploration in 3D reasoning and scene understanding.

% XW: below could be moved to related work if needed
% Notable examples include CLIP~\cite{radford2021learning}, which achieves strong performance on image classification by learning from web-scale image-text pairs, and LLaVA~\cite{liu2023llava}, which can engage in free-form dialogue about images and videos. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/teaser_v2.pdf}
    \caption{
    \ours and 3D-grounded reasoning. The task requires a model to understand the input text prompt and ground it in 3-dimensional space. 
    % Example 3D reasoning task. 
    % \yy{initial draft, to be updated, the figure need to be replaced.} 
    % \vc{Perhaps we need 2 images. On left, we have original image without box, and right we have an image (with alpha =0.5) and box overlayed. I will make the two images. Also, the scene may be too simple?} 
    }
    \label{fig:teaser-figure}
    % https://drive.google.com/file/d/1XI8jVeHNZ0SYOOQdBUPD3DK8dJeLQ5ob/view?usp=sharing
\end{figure}
% - As MMFMs show incredible capabilities in reasoning, we seek to adapt the large-scale pre-trained MMFMs to enhance the reasoning capability for autonomous driving systems. Different from language and 2D vision tasks that typical MMFM models are pretrained on, in order to fully leverage the reasoning capability of MMFMs, we will first need to adapt them to understand the elements in 3D.

% Recognizing this gap, in this work, we seek to adapt these large-scale \mmfm{}s to enhance the reasoning in 3D for autonomous driving systems, and focus on the 3D grounding and the 3D QA task to validate the 3D reasoning ability.
% Unlike the typical language and 2D vision tasks that \mmfm{}s are already pre-trained on, adapting them for 3D reasoning requires a fundamental shift. 
% The most naive way of adapting 2D-based \mmfm{}s is to directly fine-tune them on the 3D grounding or QA task. However, as shown in ??\yy{ref to the result table}, direct fine-tuning yields sub-optimal results.
% We hypothesise that this is due to that the elements of the 3D world -- depth, spatial relationships, and the dynamic nature of objects -- are not present in 2D vision or natural language data that typical \mmfm{}s are pre-trained on. \yc{do we need to emphasize the importance of 3D in the AV context?}

\textbf{Contributions:} Towards this end, our work aims to enhance \mmfm{}s' capabilities for 3D reasoning, specifically focusing on AV applications. To do so, we propose four key contributions:
\begin{enumerate}
    \item A large-scale 3D visual-language pretraining dataset (\dataset{}) constructed by merging numerous 2D and 3D datasets set both indoors and outdoors, applying heuristics to generate diverse grounding tasks for \mmfm{} pretraining to improve 3D grounding and reasoning.
    \item Visual Chain-of-Thought Prompting to connect 2D semantic reasoning with 3D scene geometry understanding for enhanced 3D grounding, employing high-resolution finetuning to boost overall performance significantly.
    \item A model-agnostic method for injecting specialist models to utilize diverse input modalities effectively.
    \item Evaluations on talk2car and Drive-LM for both 3D grounding and reasoning, achieving significant improvements over baselines by 7 and X points respectively.
\end{enumerate}

\boris{everything after here is quite detailed for an introduction and should be moved to method or even experimental sections.}

% a new large-scale 3D vision-language pre-training dataset that integrates object grounding tasks across both 2D and 3D domains. In addition to aggregating a variety of large-scale 2D grounding datasets such as COCO~\cite{}, RefCOCO~\cite{}, and O365~\cite{}, we generate an extensive set of 3D question-answer pairs for object grounding by leveraging human annotations from 3D detections \yy{correct it if this is wrong} and find that it significantly enhances alignment between 3D information and natural language.

% focusing on the 3D grounding and 3D visual question-answering tasks.
An immediate and straightforward approach for adapting these models is to fine-tune them on tasks of 3D grounding or 3D question answering. However, as we will show in \cref{sec:expts},
% our experiments indicate (Sec. ??\yy{ref to the result table}),
fine-tuning alone yields sub-optimal performance.
% We hypothesize that this is because essential 3D attributes such as depth, spatial relationships, and the motion dynamics of objects, are largely absent in the 2D vision and language datasets on which existing \mmfm{}s are pre-trained. 
Instead, we argue there is a need for a methodological shift in adapting existing \mmfm{}s for 3D reasoning tasks.
% \yc{do we need to emphasize the importance of 3D in the AV context?}

To validate our hypothesis, we first developed a large-scale 3D vision-language pre-training dataset that integrates object grounding tasks across both 2D and 3D domains. Specifically, our dataset is built on top of the Omni3D dataset~\cite{brazil2023omni3d}, which encompasses a diverse set of indoor and outdoor scenes, originally curated for 3D object detection tasks. \yy{We also includes 3D data from nuScenes, right?}
% This dataset converts all images to a virtual camera format with uniform intrinsic properties. \yy{is it necessary detail for intro?}
To tailor the dataset for \mmfm{}s pre-training, we generate an extensive set of 3D question-answering pairs for object grounding by leveraging the human annotations from 3D detections \yy{correct it if this is wrong}, which significantly enhances the model's capabilities in aligning 3D information with natural language.
% , particularly in comprehending depth. 
% Additionally, we show our \mmfm{}s demonstrate favorable scaling laws with respect to the dataset size. 
Our dataset is also augmented with a variety of large-scale 2D grounding datasets such as COCO~\cite{lin2014microsoft}, refCOCO~\cite{refcoco}, and Objects365~\cite{o365}, to improve the model's ability to generalize across various scenes and foster a more robust understanding of both 2D and 3D contexts. 

% XW: this sounds like the parts we should put into the last paragraph in the intro for the results highlights/summary
% Pre-training our \mmfm{} on this combined large scale dataset consistently enhances its performance on downstream tasks, shown in section [], and the model scales nicely with respect to the dataset size.

% This pre-training dataset integrates 2D and 3D grounding tasks to enhance both 2D semantic reasoning and depth perception. However, it lacks a mechanism to incorporate 2D capabilities to further boost 3D grounding performance. 
% To address this gap, we introduce a Chain-of-Thought (CoT) 3D grounding method, by first estimating the bounding box on 2D images based on the language question.
% Though the combined pre-training dataset integrates both 2D and 3D grounding data, the 2D part still takes a larger portion and thus the model naturally performs better on 2D grounding tasks. \yy{Correct this if it is wrong}
While our dataset integrates both 2D and 3D grounding data, the predominance of 2D data means the model is naturally more adept at 2D grounding tasks. \yy{Correct this if it is wrong}
To ease the difficulty of directly reasoning in 3D and fully leverage the model's well-trained 2D reasoning capability, we introduce a Visual Chain-of-Thought Prompting to improve 3D grounding result. 
CoT first estimates the bounding box on 2D images based on the language question, then prompts the model with the predicted 2D bounding box to estimate the corresponding 3D bounding box. 
% This approach effectively breaks down the challenging 3D grounding task into tasks of 2D semantic reasoning and 3D depth estimation, 
% allowing for better utilization of 2D understanding and simplifying the process of understanding 3D space. 
By decomposing the complex 3D grounding task into more manageable sub-tasks of 2D semantic reasoning followed by 3D depth estimation, we facilitate a more effective use of the model's 2D proficiency to enhance its understanding of 3D spaces.
% Moreover, we highlight the importance of higher image resolution that significantly boosts the accuracy of long-range depth estimation, leading to improved 3D grounding. 
Additionally, we underscore the significance of high image resolution in improving the accuracy of long-range depth estimation, which is crucial for precise 3D grounding.
% We first pre-train and fine-tune our \mmfm{} on low-resolution images, then further fine-tune it on high-resolution images. 
Our training approach involves an initial pre-training and fine-tuning phase using low-resolution images, followed by further fine-tuning on high-resolution images.
These two techniques yield consistent performance improvement on both 3D grounding and QA tasks.

To expand the input modalities, we propose a model-agnostic approach that utilizes predictions from specialized models utilizing different modality, \eg, LiDAR-based 3D object detection models.
The predictions from specialized models serve as supplementary information to the original question for 3D grounding. 
We train the model with the ground truth of the specialized task and incorporate specialized models' output during interference, ensuring it remains independent of any specific models.

We evaluate our model's performance in both 3D grounding and 3D reasoning on various autonomous driving datasets. 
In the case of 3D grounding, our evaluation on the \ttc dataset~\cite{deruyttere2019talk2car} shows that our model surpasses the baseline models by 7 points in Bird's Eye View (BEV) accuracy and by 5 points in 3D\yc{It's hard to tell the improvement without knowing the baseline performance}. Additionally, we have adapted the \dLM model for 2D grounding to 3D and evaluated its performance, where it exceeds the LLava fine-tuning baseline by X points. Regarding 3D reasoning, our analysis on \dLM demonstrates that our model achieves an improvement of X points over the baseline. \yc{I think evaluation-wise we might need to associate some takeaways to make this sound more exciting}


==> sections/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Vision Language Models} 
% \yy{Looks like we are using VLM and MMLM interchangeably?}
By scaling up pre-training on the internet-scale dataset, there has been significant progress for VLMs in the 2D vision-language domain, showing strong capabilities in few-shot generalization. VLBRRT~\cite{vlbert} and ViLBERT~\cite{lu2019vilbert} capitalized on a BERT-style framework for image-text co-embedding. CLIP~\cite{radford2021learning} embedded images and text captions into a shared feature space via contrastive learning and pioneered zero-shot vision tasks. BLIP~\cite{li2022blip} and BLIP2~\cite{Li2023BLIP2BL} further improved CLIP by leveraging extra pseudo-labeled data and better image/language encoders. Flamingo~\cite{Alayrac2022FlamingoAV} and its open-source implementation Open-Flamingo~\cite{Awadalla2023OpenFlamingoAO} proposed a fast adaptation approach to enable in-context few-shot learning on novel visual-language tasks. GPT4V~\cite{Achiam2023GPT4TR} and Gemini~\cite{team2023gemini} further demonstrated state-of-the-art human-level visual reasoning ability through scaling. LLaVA~\cite{liu2023llava} pioneered instruction fine-tuning in the multimodal field. Unified-IO2~\cite{lu2023uio2} scaled autoregressive multimodal models with vision, language, audio, and action. However, these works have predominantly focused on the 2D vision and language tasks and 
not tackled complex 3D reasoning tasks. 
% had limitations in complex 3D reasoning. 
We aim to adapt these \mmfm{}s to enhance their capabilities for complex 3D reasoning in long-tail scenarios. 
% In summary, visual language models have been largely advanced by scaling models with large data, leading to strong few-shot generalization to visual data.   

\subsection{Image-grounded Reasoning}
With the advancement of multi-modal large language models, image-grounded reasoning (referring and grounding) has shown a great progress in 2D space.
Image-grounded reasoning requires a model to localize an object or a region that an input prompt enquires, or describe about a region of interest. 
VisionLLM~\cite{wang2024visionllm} adapts 2D object detector to align with an LLM, and GPT4-ROI~\cite{zhang2023gpt4roi} employs hierarchical feature modeling of detectors to reason about input visual prompt (ROI). 
Kosmos-2~\cite{peng2023kosmos} and Shikra~\cite{chen2023shikra} have shown pure transformer-based visual encoder can surpass using 2D detectors with data scaling. 
Recently, Ferret~\cite{you2023ferret} have shown remarkable image-grounded reasoning from both free-form visual prompt and text prompt. 
These works mainly consider reasoning in 2D space (image coordinate), and our work expands the reasoning capability to 3D space (camera coordinate) for the first time. 

\subsection{\todo{VLM for AV doesn't fit anymore}}

% \subsection{Reasoning with Language Models in Autonomous Driving} 

% Reasoning is a long-standing problem in autonomous driving. GPT-Driver~\cite{mao2023gpt} incorporated reasoning into autonomous driving by reformulating motion planning as a language modeling problem and introducing fine-tuned LLMs as a motion planner. DriveGPT4~\cite{xu2023drivegpt4} proposed an end-to-end driving approach that leverages a vision language model to directly predict actions from sensory inputs. DiLu~\cite{wen2023dilu} capitalized on a knowledge-driven approach with large language models to improve reasoning capability. Agent-Driver~\cite{mao2023language} proposed an LLM-based embodied agent, achieving state-of-the-art decision-making performance and making it transparent. Dolphins~\cite{ma2023dolphins} proposed an instruction fine-tuning pipeline for \mmfm{}-based autonomous driving. DriveLM~\cite{sima2023drivelm} opted to use graph visual question answering to tackle reasoning problems in autonomous driving. LMDrive~\cite{shao2023lmdrive} tackled closed-loop autonomous driving with language models. Our method is closely related to these prior works since we attempt to solve visual reasoning problems in autonomous driving. In contrast to prior work, \ours{} can directly reason in the 3D space for complex AV perception scenarios, and can be trained in an end-to-end fashion. 

% In this work, we empower the \mmfm{}-based AV pipeline... by explicit grounding the \mmfm in 3D.


% \yue{say something special about our method}



% \subsection{Unifying Camera Parameters\yue{why should we discuss camera parameters? }}

==> sections/3_method.tex <==
\section{Unified Language-Image Pretraining for 2D and 3D}
\label{sec:method}

Our goal is to expand the capabilities of vision-language models to reason in 3-dimensional space. 
We propose a unified training framework to learn from both 2D and 3D perceptual data as well as standard image-text pairs. 
In this section, we first discuss about data standardization to train a vision-language model at scale (Sec.~\ref{sec:data_scale}), {task scaling} for reasoning about perceptual information in versatile I/O format (Sec.~\ref{sec:task_scale}), \textit{visual chain-of-thought} reasoning for 3D grounding and question answering tasks (Sec.~\ref{sec:v_cot}), and finally, we present \ours, the final model of our unified training framework built on LLaVA-1.5~\cite{liu2023improvedllava} (Sec.~\ref{sec:arch}). 
% We further apply high-resolution finetuning to improve the long range object grounding and model agnostic 


\subsection{Data-scaling for Image-based 3D Reasoning}
\label{sec:data_scale}
The main challenge of training from image-based 3D data is the difference in sensor configurations. 
\emph{Specialist} vision models design their network architecture and learning objective specific to dataset-level sensor configurations (\textit{e.g.,} Bird's-Eye-View representation).  
Such customization of model architecture excels in target tasks but limits scalability of general-purpose models. 
Instead, we explore the limit of training a \textit{generalist} model with pure data-scaling. 
To this end, we combine a large collection of 2D and 3D vision datasets from different camera intrinsic and formulate the problem 
as a \textbf{next token prediction} task. 


\vspace{0.2cm}\myparagraph{Data standardization.} 
% \todo{This subsection needs a rewrite.}
We consider points and boxes as our main spatial representation for 2D and 3D reasoning. 
We convert every label to either a point $o^{\text{2D}}_{\text{point}}=[\hat{x}, \hat{y}]$ or a bounding box $o^{\text{2D}}_{\text{box}}=[\hat{x}, \hat{y}, \hat{x}', \hat{y}']$.
Similarly, we convert every 3D label to either 
$o^{\text{3D}}_{\text{point}}=[{x}, {y}, z]$ or  $o^{\text{3D}}_{\text{box}}=[{x}, {y}, z, w, h, l, r_1, r_2, r_3]$ where $r_1$, $r_2$, $r_3$ are Euler angles. 
We first standardize image-based 3D datasets by unifying camera parameters. 
We follow the procedure of Omni3D~\cite{brazil2023omni3d}; define a virtual camera with a fixed focal length $f$ and transform depth $z$ according to the original camera parameters and the target image size. 
Since all 3D labels are unified to a consistent camera intrinsic, we can now convert all x and y coordinates to 2D projected coordinates ($\hat{x}, \hat{y}$). 
Consequently, we can represent all label formats to naturally follow 2D to 3D per-object token sequence: 
\begin{align}
    o^{\textcolor{mytangoblue}{\textbf{2D}}}_{\text{point}} &= [\textcolor{mytangoblue}{\hat{x}}, \textcolor{mytangoblue}{\hat{y}}] \\
    o^{\textcolor{mytangoblue}{\textbf{2D}}}_{\text{box}}\ \;   &= [\textcolor{mytangoblue}{\hat{x}}, \textcolor{mytangoblue}{\hat{y}}, \textcolor{mytangoblue}{\hat{x}'}, \textcolor{mytangoblue}{\hat{y}'}] \\
    o^{\textcolor{myred}{\textbf{3D}}}_{\text{point}} &= [\textcolor{mytangoblue}{\hat{x}}, \textcolor{mytangoblue}{\hat{y}}, \textcolor{myred}{{z}}] \\
    o^{\textcolor{myred}{\textbf{3D}}}_{\text{box}} \ \;  &= [\textcolor{mytangoblue}{\hat{x}}, \textcolor{mytangoblue}{\hat{y}}, \textcolor{myred}{{z}}, \textcolor{myred}{{w}}, \textcolor{myred}{{h}}, \textcolor{myred}{{l}}, \textcolor{myred}{{r}_1}, \textcolor{myred}{{r}_2}, \textcolor{myred}{{r}_3}]
\end{align}
where each value is represented as a short sequence of text tokens (5 for 3-decimal numbers). 
This allows the model to predict consistent ordering of token sequence from 2D to 3D, which improves the understanding of the underlying structure.
With autoregressive models, we first localize objects in image coordinates ($\hat{x}, \hat{y}$), then infer depth ($z$), and then infer the size and orientation ($w,h,l,r_1,r_2,r_3$).

% \todo{Motivate this more clearly. Human perceives objects this way too. We localize in retina to focus, estimate depth, and understand the size and orientation from the appearance. Or we can go the other way around; depth requires a point to estimate, size needs depth, etc. Also, no y for output. }

% This also lets the model to infer normal 2D-based grounding without known camera parameters. 


\vspace{0.2cm}\myparagraph{3D reasoning as multi-turn conversations.}
Now, we combine the 2D and 3D data with language-image instruction tuning data of visual language models~\cite{liu2023llava}.
For each image and a set of object labels pair, we construct a multi-turn conversational question-answer data (\textbf{Q}$_1$, \textbf{A}$_1$, \textbf{Q}$_2$, \textbf{A}$_2$, $\dots$, \textbf{Q}$_n$, \textbf{A}$_n$). 
Each question refers an object with one property $b_q$ and enquires $b_a$:
\begin{align}
b_q, b_a \in \{\text{box}_\text{2D}, \text{caption}, \text{box}_\text{3D}\} 
\end{align} 
Each object property has a set of {prompts} predefined, such as \texttt{``Provide the 3D bounding box of the region this sentence describes: <caption>''} for $b_q=\text{caption}$ and $b_a=\text{box}_\text{3D}$.
We combine the meta information of objects (e.g., attribute, physical state, etc.) with the class name to enrich the textual information.


% \begin{enumerate}
%     \item Standarize localization as a sequence of tokens.
%     \item Predict the projected centers in 2D coordinates and rescale depth with respect to image size and a fixed virtual camera (cite omni3d). 
%     \item Normalize across datasets and map the values into 1000 bins. 
% \end{enumerate}

\subsection{Task-scaling for Versatile I/O Format}
\label{sec:task_scale}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/dataset_v4.pdf}
    \caption{\textbf{Task-scaling for versatile I/O format.} Decomposing the existing label formats for 3D grounding task. A complete 3D location can be decomposed into a center point (\texttt{[x, y, z]}), a depth (\texttt{[z]}), a (projected) 2D point (\texttt{[x$_\text{c}$, y$_\text{c}$]}), and a (projected) 2D box (\texttt{[x1, y1, x2, y2]}). We define various tasks that connect among these to train versatile I/O formats. \textbf{Left}: available (decomposed) annotations. \textbf{Right}: various tasks for training. }
    \label{fig:tasks}
    \vspace{-0.5cm}
    % https://drive.google.com/file/d/1XI8jVeHNZ0SYOOQdBUPD3DK8dJeLQ5ob/view?usp=sharing
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/method_v4.pdf}
    \vspace{-0.2cm}
    \caption{\textbf{\ours inference}. \textbf{Left}: Visual Chain-of-Thought Prompting to reason in 3D step-by-step. \textbf{Right}: Incorporating specialist models to further improve localization of \ours. 
    Our model can either predict directly from text prompt, or with visual chain-of-thought prompting or specialist prediction as prompts. 
    }
    \label{fig:method}
    % \vspace{-0.5cm}
    % https://drive.google.com/file/d/1XI8jVeHNZ0SYOOQdBUPD3DK8dJeLQ5ob/view?usp=sharing
\end{figure}

We are interested in a generalist model that accepts input and generates     output in versatile formats.
Users may want to supplement 2D points or boxes as visual prompt during inference, or may only want the metric depth of an object instead of a complete 3D location. 
This interest in versatile I/O format shares the same spirit of instruction tuning in 2D-based visual language models~\cite{liu2023llava,Dai2023InstructBLIPTG,Alayrac2022FlamingoAV}. 
To this end, we define multiple relevant tasks for a model to adapt to wider spectrum of similar tasks in 2D and 3D. 
We start by \emph{decomposing} the existing label formats to easier tasks as illustrated in Figure~\ref{fig:tasks}. 
After, we have expanded set of object properties to construct question-answer pairs:
\begin{align}
b_q &\in \{ \text{point}_\text{2D}, \text{box}_\text{2D}, \text{caption}, \text{point}_\text{3D}, \text{box}_\text{3D} \} \\
b_a &\in \{\text{point}_\text{2D}, \text{box}_\text{2D}, \text{caption}, \text{depth}, \text{point}_\text{3D}, \text{box}_\text{3D} \} 
\end{align}
We construct up to $n=30$ question answer pairs $(\textbf{Q}^{b_q}_{b_a},\textbf{A}_{b_a})$ sampled at random for each data. 
We combine a collection of 2D and 3D vision datasets (\dataset{}), summarized in Table~\ref{tab:dataset_summary}, and jointly train with this expanded set of tasks.
Note that Omni3D~\cite{brazil2023omni3d} contains front-camera images of NuScenes~\cite{nuscenes2019} dataset; we supplement with images from all camera orientations after excluding scenes in validation splits of \ttc and \dLM. 


% \todo{talk about \dataset{}}

% \begin{enumerate}
%     % \item Training 3D reasoning directly is hard. 
%     % \item 3D reasoning can be decomposed into ``easier'' tasks.
%     % \item Also allows model to take more versatile input and output format. (same as instruction tuning) 
%     \item Exhibit greater scalability during training regardless of data scale. 
%     \item Allows not only text prompting but also visual prompting (points and boxes). 
% \end{enumerate}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/method_v4.pdf}
%     \vspace{-0.2cm}
%     \caption{\textbf{\ours inference}. \textbf{Left}: Visual Chain-of-Thought Prompting to reason in 3D step-by-step. \textbf{Right}: Incorporating specialist models to further improve localization of \ours. 
%     Our model can either predict directly from text prompt, or with visual chain-of-thought prompting or specialist prediction as prompts. 
%     % \yy{to update the LiDAR screenshot}
%     }
%     \label{fig:method}
%     \vspace{-0.5cm}
%     % https://drive.google.com/file/d/1XI8jVeHNZ0SYOOQdBUPD3DK8dJeLQ5ob/view?usp=sharing
% \end{figure}
% \subsection{Visual Chain-of-Thought Prompting}
% \label{sec:v_cot}



\subsection{Visual Chain-of-Thought Prompting}
\label{sec:v_cot}

One of the most intriguing properties of large language models is its \emph{emergent} ability to improve reasoning with intermediate steps~\cite{wei2022chain}.
This mostly attributes to vast corpus of rich text data with numerous step-by-step question answering samples~\cite{wei2022finetuned}. 
We artificially supplement this \emph{step-by-step} reasoning of 3D by interleaving multiple questions of the same object from easy-to-hard order (the left part of Figure.~\ref{fig:method}): 
\begin{align}
\text{maximize} \quad 
\begin{cases}\quad 
    p(\text{\textbf{A}}_{\text{box}_\text{2D}}|\textbf{Q}^{\text{caption}}_{\text{box}_\text{2D}}) & \textit{question 1} \\ \quad p(\text{\textbf{A}}_{\text{box}_\text{3D}}|\textbf{Q}^{\text{caption}}_{\text{box}_\text{2D}},\text{\textbf{A}}_{\text{box}_\text{2D}},\textbf{Q}^{\text{caption}}_{\text{box}_\text{3D}}) & \textit{question 2} \\
    \quad \quad ...
\end{cases}
\end{align}
Furthermore, we allow test-time adaptation to any specialist models by mixing in \emph{candidate} objects as a system prompt (the right part of Figure.~\ref{fig:method}). 
This effectively alleviates the problem of localizing in 3D to ``choosing the appropriate box from candidates'',
\begin{align}
\text{maximize} \quad p(\text{\textbf{A}}_{\text{box}_\text{3D}}|\textbf{S}_{\text{box}_{\text{3D}}}, \textbf{Q}^{\text{caption}}_{\text{box}_\text{3D}})
\end{align}
where \textbf{S}$_{\text{box}_{\text{3D}}}$ is a set of candidate boxes, which can be provided by any specialist models (depending on available input modalities) at inference. 
During training, we use the ground truth boxes with a prompt \texttt{``Here is the list of 3D bounding boxes of all objects around the camera:''} and our model does not bind with any particular specialist model. 


% \begin{enumerate}
%     \item Directly inferring 3D can be hard and ill-defined. 
%     \item We train with interleaving questions of 3D 
%     \item For 3D QA, we also train with interleaving questions 
%     \item Improve reasoning by allowing the model to go step-by-step. 
% \end{enumerate}


\subsection{\ours}
\label{sec:arch}

We introduce \ours, a language-image model based on LLaVA-1.5 architecture trained to reason in both 2D and 3D. 
Although we maintain the generality of model architecture, we make simple yet critical changes to the original LLaVA. 
We first replace the CLIP visual encoder with DINOv2~\cite{oquab2024dinov}, and undergo the same alignment step of the original LLaVA. 
Although DINOv2 is not a text-aligned visual encoder like CLIP, we found minimal degradation in the standard visual language model benchmarks while significantly improving 3D-related tasks. 
Then, we finetune the language model (Vicuna-7B~\cite{vicuna2023}) while freezing the visual encoder and jointly on LLaVA instruction-following data and our collection of data following Sec.~\ref{sec:data_scale},~\ref{sec:task_scale} and~\ref{sec:v_cot}. 
We use low image resolution ($336 \times 336$) and train with a large batch size. 
Then, we add an additional finetuning stage for both visual and language models with high resolution images ($672 \times 672$). 
% \vc{This may go to implementation detail.}

==> sections/4_results.tex <==
\section{Experiments}
\label{sec:expts}


\todo{Pretrained model (wo finetune) on Omni3D, scaling plot, with and without step-by-step, 2D only vs 3D pretrain (in finetune case), stage wise (2D -> 3D) vs all same (2d+3d ->2d+3d).}

We evaluate the effectiveness of \ours in three aspects: (1) 3D-grounded reasoning, (2) complex reasoning in 3D, and (3) standard vision-language benchmark (POPE~\cite{Li-hallucination-2023}). 
% \vspace{-0.5cm}
\subsection{Implementation Details}
We use LLaVA-1.5 \cite{liu2023improvedllava} with Vicuna-7B as our base model. 
We replace the CLIP visual encoder with ViT-L/14~\cite{dosovitskiy2020vit} based DINOv2. 
For all localization outputs, we use 3 decimal places with text tokens, and keep 5 tokens per value (e.g., \texttt{[0.120, 0.521, ...]}). 
Accordingly, we pre-process all LLaVA instruction-following data to reflect this change. 
We follow the same alignment step to train the MLP projection layers with the same training setup in\cite{liu2023improvedllava}. 
For 2D and 3D pretraining, we use random sampling following the sampling rate in Table~\ref{tab:dataset_summary}. 
Each data sample (image-annotation pair) is converted to the multi-turn conversation format (Fig.~\ref{fig:tasks}) sampled at random. 
During pretraining, we use 8$\times$8 A100s with a batch size of 1024 and train the model with a learning rate $lr=10^{-4}$ on images with $336 \times 336$ resolution. 
Then, we fine-tune all parameters including the visual encoder on a higher resolution $672 \times 672$ with 8 A100s and a batch size of 32$\times$4 (effective batch size of 128 with 4 gradient accumulation steps) and a learning rate $lr=2\times 10^{-5}$.

\input{tables/dataset_stats}

\subsection{Datasets}

\todo{Omni3D for evaluation, VLM benchmark data, etc.}

We pre-train \ours on \dataset{}, and then fine-tune it on the training split of the target datasets, \ttc and \dLM.

\myparagraph{\ttc}~\cite{deruyttere2019talk2car} is a 3D referring expression comprehension dataset of various driving scenarios. 
It consists of 8,349 training samples and 1,163 validation samples with images and LiDAR data. 
It provides rich question-answer pairs grounded to an object in the image. 
Each object is labeled with a situational text that uniquely identifies the object (e.g., ``\textit{Wow hold on! That looks like my stolen bike over there! Drop me off next to it.}''). 
The original benchmark~\cite{deruyttere2019talk2car} evaluates the 2D grounding performance with the AP$_{0.5}$ metric. 
MSSG~\cite{cheng2023language} extends the task to 3D grounding and evaluates on both BEV AP and 3D AP.
% , with two different sets of IoU thresholds A and B, where B is more strict overall than A. 


\myparagraph{\dLM}~\cite{sima2023drivelm} is a recently released question-answering dataset for autonomous driving based on the nuScenes dataset~\cite{nuscenes2019}.
It consists of various driving scenes with multi-view images and LiDAR point clouds, as well as frame-level question-answering data, and has a total of $4871$ frames. 
Each frame contains 91.4 question-answer pairs on average, covering core autonomous driving tasks such as perception, prediction, and planning, as well as a short description and 2D boxes of important objects.  
To evaluate \ours, we construct another 3D grounding benchmark based on the \dLM dataset, which we call \textbf{\dLM-Grounding}.
We associate the 2D boxes with the nuScenes 3D bounding boxes by computing the IoU between 2D boxes projected from 3D labels and the 2D boxes of labeled important objects, and only keep those with a IoU greater than $0.35$. 
After association, \dLM-Grounding has a total of 13,287 images, about one annotation per image. 
We also use the \textbf{\dLM-QA} data from the original {\dLM} to fine-tune \ours for complex reasoning tasks.
The original training split has 696 scenes in total. 
We use 600 scenes for training and 96 scenes for validation, which we include the \dLM provided scenes for sample evaluation and \ttc validation split scenes. 
% \todo{how many images in DriveLM-Grounding, DriveLM QA evaluation metric}
We evaluate 3D grounding with the same BEV AP and 3D AP metric as those in \ttc. 



\subsection{3D-Grounded Reasoning}


% DriveLM also includes descriptions of each object with the 2D box and physical state. 
% We repurpose this dataset as 3D grounding dataset by associating the 2D boxes with 3D boxes from NuScenes, and pair each object with the description.

\input{tables/talk2car_grounding}
\input{tables/drivelm_grounding}

\input{tables/rec}
\input{tables/mllm_bench}

\input{tables/data_scaling}


\input{tables/ablation_two_tables}


Our results for 3D grounding on the \ttc dataset are detailed in Table \ref{tab:talk2car_main}, which is structured according to the input modalities used for 3D grounding. 
The baselines that rely solely on camera inputs are only evaluated on 2D grounding, whereas those incorporating both camera and LiDAR inputs are evaluated on both 2D and 3D grounding. \ours is pre-trained on \dataset{} and fine-tuned on \ttc with resolution $672 \times 672$. We apply visual Chain-of-Thought when predicting the 3D grounding.
Remarkably, our camera-only \ours significantly surpasses the state-of-the-art model FA~\cite{fa} by 5.7 points on 2D AP$_{0.5}$. Surprisingly, \ours also outperforms the camera+LiDAR baseline, \ttc-3D~\cite{deruyttere2019talk2car}, by 15.7 points on the BEV AP$_\text{A}$ metric. 
Our camera-only \ours is only 3.8 points behind the state-of-the-art camera+LiDAR baseline MSSG~\cite{cheng2023language}. 
MSSG~\cite{cheng2023language} utilized the outputs of the pre-trained CenterPoint model~\cite{yin2021center} for predicting 3D grounding. Similarly, we leverage the LiDAR modality by using the predictions from CenterPoint~\cite{yin2021center}, selecting the top-30 boxes with the highest confidence as a visual prompt.
We observe a substantial 17.8 points improvements, outperforming MSSG~\cite{cheng2023language} by 7.4 points. 
Furthermore, We observe a similar trend on the \dLM-Grounding dataset, shown in Table~\ref{tab:drivelm_main}. 
Similar to \ttc, \ours shows significant improvements compared to directly finetuning from LLaVA-1.5, resulting in a 32.8 points improvement on the BEV AP$_\text{A}$ metric. 


\subsection{Complex Reasoning in 3D}
\input{tables/drivelm_qa}
To show the effectiveness of 3D reasoning capability, we finetune \ours on \dLM-QA dataset. 
The dataset comprises questions about \textit{perception} (e.g., ``what are the objects worth noting in the current scenario?''), \textit{prediction} (e.g., ``where might the van, the sedan, and the pedestrian move in the future?), \textit{planning} (e.g., ``what are the safe actions of the ego car considering those objects?'') and \textit{behavior} (e.g., ``what would the ego vehicle's next action would be?''). 
We compare \ours with LLaVA-1.5~\cite{liu2023improvedllava} to show the impact of our pretraining, as well as the official baseline~\cite{sima2023drivelm} that has been recently released.
All models use 7-B scale LLM (Vicuna-7B~\cite{vicuna2023} or LLaMA-7B~\cite{touvron2023llama1}) and are fine-tuned on subset of \dLM train split. 
Top rows are the result on scenes held out by the authors and bottom rows are our additional split to evaluate models on a larger testset. 
The evaluation metric is based on accuracy, match (localization), BLEU/CIDEr, and ChatGPT score for favorable text generation. 
In both setting, \ours show competitive result consistently. 

\subsection{Ablation Study}
Our work consists of three key contributions, including a large-scale language-visual pre-training dataset~\dataset{}, visual chain-of-thought prompting, and specialist prompting. We provide comprehensive ablation studies for each of our design choices for \ours.

\vspace{0.2cm}\myparagraph{Data-scaling effect.} 
\dataset{} combines seven datasets, cumulatively encompassing 1.1 million images. To illustrate the impact of data-scaling on the performance, datasets are incrementally integrated during pre-training stage. We employ \ours without Visual Chain-of-Thought (VCoT) and fine-tune it at the image resolution $336 \times 336$. The results are presented in Table~\ref{tab:dataset_performance}. We observe a consistent improvement in performance, where AP grows from 19.7 to 44.7, improving by 126\%. It is also noteworthy that the incorporation of 2D data during pre-training benefits the model, even though the fine-tuning is performed for 3D grounding tasks - we observe a significant 37\% performance gain after including  refCOCO and COCO.

\vspace{0.2cm}\myparagraph{Visual Chain-of-thoughts (VCoT) prompting during inference.} We evaluate \ours on \ttc with and without VCoT. As shown in Table~\ref{tab:vcot_ablation}, employing VCoT prompting yields significant enhancements in performance, with a improvement of (+6.2\%, +6.7\%, +6.1\%, +14.4\%) observed. 
It demonstrates that our VCoT is able to effectively bridge the gap between 2D semantic reasoning and 3D geometry reasoning. 


\vspace{0.2cm}\myparagraph{Impact of specialist prompting during inference.} 
Specialist prompting can leverage new input modality, such as LiDAR. 
As demonstrated in Table~\ref{tab:talk2car_main} on \ttc dataset, employing CenterPoint~\cite{yin2021center} predictions as visual prompts significantly improves the performance of \ours with gains of (+24.2\%, +46.2\%, +47.8\%, +58.2\%) in 3D grounding. 
Note that \ours needs neither CenterPoint nor LiDAR points during training, which means user can choose any specialist model based on the available input modality. 
% However, it is noteworthy that there is a minor decrease of 0.5\%  in 2D grounding performance, which could potentially be attributed to randomness in the training process. 


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.963\linewidth]{figures/cot_visualization.pdf}
    % \vspace{-2.5em}
    \caption{\textbf{Visualization} of \ours prediction on unseen scenes of Talk2Car dataset. We show the original image (left), 2D prediction (middle), and 3D prediction (right). The input prompt is under each row. }
    \label{fig:cot_visualization}
\end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/omni3d_vis.pdf}
    \vspace{-0.2cm}
    \caption{\textbf{Visualization} of \ours prediction on indoor objects. Although our primary focus is on outdoor objects, \ours is also capable of localizing indoor objects. The text prompts/ class names are ``sofa'', ``book'', ``chair'', ``laptop'', ``bottle'', ``trash bin'', ``chair'', and ``bottle.'' }
    \label{fig:omni3d_vis}
    \vspace{-0.5cm}
\end{figure}

\subsection{Qualitative Results}


In Figure~\ref{fig:cot_visualization}, we show \ours prediction results of 2D and 3D grounding on unseen scenes in \ttc dataset and demonstrate that \ours is capable of reasoning complex text prompt.
For example, \ours is capable of recognizing and reasoning in 3D for ``a man in the yellow hat'' from several people present in the scene, ``a guy wearing a white shirt'' from multiple people standing in front of the car, or ``white van left of the black car'' from a number of vehicles in the parking lot.  
Further, with Omni3D~\cite{brazil2023omni3d} included in the pre-training dataset \dataset{}, we show in Figure~\ref{fig:omni3d_vis} that \ours is also capable of localizing objects in indoor scenes.
% , we show that \ours is also capable of localizing objects in indoor scenes, thanks to Omni3D~\cite{brazil2023omni3d}. 






% \subsection{downstrema SFT}

% \paragraph{Grounding}
% \begin{enumerate}
%     \item Talk2Car (Camera + LiDAR): 3D grounding outdoor
%     \item Rank2Tell (Camera + LiDAR): 3D grounding outdoor
%     \item ReferKITTI (Camera + LiDAR): 3D grounding outdoor
%     \item ReferIt3D (Camera + LiDAR): 3D grounding indoor
%     \item ScanRefer (Camera + LiDAR): 3D grounding indoor 
%     \item Omni3D (Camera): open-vocabulary 3D detection / grounding 
% \end{enumerate}

% \paragraph{QA}
% \begin{enumerate}
%     \item nuscenes QA (Camera + LiDAR): outdoor QA 
%     \item driveLM (Camera + LiDAR): outdoor QA 
%     \item scanQA (Camera + LiDAR): indoor QA 
% \end{enumerate}

% \paragraph{Specialists}
% \begin{enumerate}
%     \item BEVFormerV2 - multi-view stream outdoor   
%     \item CenterPoint - LiDAR outdoor  
%     \item PointNet2 + VoteNet - RGBD indoor 
% \end{enumerate}

% \paragraph{}


% \paragraph{MLLM benchmarks}
% \begin{enumerate}
%     \item 2D grounding (refCOCO, FLICKR, etc.)
%     \item VQAv2, textQA, POPE
%     \item MMMU
% \end{enumerate}

% \subsection{Analyses}

% \paragraph{Data scaling}
% \paragraph{Model scaling}
% \paragraph{CoT reasoning for 3D}
% \paragraph{More perception tasks help reasoning?}
% \paragraph{Quantitative results}

% \subsection{Ablations}
% \begin{enumerate}
%     \item 3D representation: direct vs log, euler vs rotation 
%     \item virtual camera vs implicit adapt 
%     \item backbone type 
%     \item training steps (backbone freeze vs finetune)
%     \item image resolution and positional encoding types 
% \end{enumerate}

==> sections/5_conclusion.tex <==
\section{Conclusion}
In this paper, we present a multi-modal language model that can reason in both 2D and 3D, named \ours. 
We provide a collection of dataset (\dataset{}) and a training framework to effectively scale \mmfm{} training for 3D understanding. 
We evaluate \ours in 3D grounded reasoning and QA tasks, and show competitive results. 
We also show that a chain-of-thought prompting further improves 3D localization of our model. 
Finally, we show that our model can adapt any specialist models during inference by prompting their predictions as visual prompts. 
We examine that pure transformer-based \mmfm{} with minimal inductive bias can learn about 3D understanding solely by data scaling. 


==> tables/ablations.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccccccc}
\hline
\textbf{High-Res} & \textbf{COT} & \textbf{SFT} & \textbf{Omni3D} & \textbf{DriveLM} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} \\
\hline
 &  &  &  &  & 35.9 & 22.3 & 25.1 & 13.9 \\
 &  \checkmark &  &  &  & 39.8 & 25.3 & 29.2 & 14.6 \\
\checkmark &  &  &  &  & 40.0 & 24.5 & 29.0 & 14.0 \\
\checkmark & \checkmark &  &  &  & 45.8 & 26.7 & 31.7 & 16.0 \\
\checkmark & \checkmark & \checkmark &  &  & 57.5 & 44.0 & 51.3 & 28.8 \\
\checkmark & \checkmark &  & \checkmark &  & 44.3 & 26.7 & 32.3 & 15.8 \\
\checkmark & \checkmark &  & \checkmark & \checkmark & 44.6 & 29.1 & 32.5 & 15.8 \\
\hline
\end{tabular}
\caption{Ablations.}
\label{table:ablations_results}
\end{table}

